Flow: Separating Consensus and Compute -- Block Formation and Execution

Most current blockchains require all full nodes to execute all tasks limits the throughput of existing blockchains, which are well documented and among the most significant hurdles for the widespread adoption of decentralized technology. This paper extends out presentation of Flow, a pipelined blockchain architecture, which separates the process of consensus on the transaction order from transaction computation. As we experimentally showed in our previous white paper, our architecture provides a significant throughput improvement while preserving the security of the system. Flow exploits the heterogeneity offered by the nodes, in terms of bandwidth, storage, and computational capacity, and defines the roles for the nodes based on their tasks in the pipeline, i.e., Collector, Consensus, Execution, and Verification. While transaction collection from the user agents is completed through the bandwidth-optimized Collector Nodes, the execution of them is done by the compute-optimized Execution Nodes. Checking the execution result is then distributed among a more extensive set of Verification Nodes, which confirm the result is correct in a distributed and parallel manner. In contrast to more traditional blockchain architectures, Flow's Consensus Nodes do not execute the transaction. Instead, Verification Nodes report observed faulty executions to the Consensus Nodes, which adjudicate the received challenges and slash malicious actors. In this paper, we detail the lifecycle of the transactions from the submission to the system until they are getting executed. The paper covers the Collector, Consensus, and Execution role. We provide a protocol specification of collecting the transactions, forming a block, and executing the resulting block. Moreover, we elaborate on the safety and liveness of the system concerning these processes.

==> preliminaries/security_terms.tex <==
\subsection{Security Terminologies}

%\note{[AlexH: I find this section quite complex and easy to get wrong. In my opinion, a formal definition of `Consensus Authenticity' is not needed for this paper as we do not develop a consensus algorithm. I think it is quite intuitive to expect that only authorized nodes are permitted to participate in consensus. If a `consensus result' is not signed by the appropriate nodes, it is simply not a consensus result but just garbage. I would recommend moving this section to the part where we talk about Collector clusters. In my opinion, Collector clusters are  the only part where we need to explicitly discuss authorization to participate in consensus.]}\bigskip

\noindent
\label{flow:subsection_security_terms}
\textbf{Consensus Authenticity:} %by all the required party
In the rest of this paper, we refer to the term \techterm{consensus authenticity} as a security measurement of the consensus result. A consensus result is authenticated if it has been signed by all the authorized nodes with the minimum required effective votes satisfied. For example, as we explain in the rest of this paper, a consensus over a collection has authenticity if it has a minimum effective vote of $\frac{2}{3}$ of the Collector Nodes of \textit{its cluster}. However, solely having the minimum effective votes does not suffice. Rather those votes should come from the authorized nodes, i.e., the nodes that have a legitimate right to participate in the consensus. 
% For a node to be authenticated on participating in a consensus over a collection, it should be (1) a Collector Node, and (2) all the transactions represented by the collection should be assigned to that node's corresponding cluster. We elaborate in detail on this topic in Section \ref{flow:sec_collection}. 
However, we would like to emphasize that not every \Architecture node is authorized to participate in a consensus of its choice. 

\bigskip
\noindent
\textbf{Consensus Integrity:} %the change in the state is done by the authenticated parties
The consensus process has integrity if all the state transitions occur solely from the authenticated nodes. In other words, starting from a publicly agreed initial $S_{0}$ state, a consensus protocol over variable $S$ is modeled as $\{S_{0}, S_1, S_2, ...\}$ where $S_{i}$ shows the $i^{th}$ state of $S$. Consensus progress then is said to have the integrity if all the state transitions $S_{i-1} \rightarrow S_{i}$ are done in an authenticated manner and by the authenticated nodes. Consensus progress over the variable $S$ is said to not have the integrity feature if there exists a state $S_{i'}$ where $S_{i'} \rightarrow S_{i'+1}$ is done in an unauthenticated manner.%https://www.overleaf.com/project/5d97bc65c4b9cc0001e30dea
